Exploring the Design of Collaborative Applications via the Lens of NDN Workspace

Metaverse applications desire to communicate with semantically identified objects among a diverse set of cyberspace entities, such as cameras for collecting images from, sensors for sensing environment, and users collaborating with each other, all could be nearby or far away, in a timely and secure way. However, supporting the above function faces networking challenges. Today's metaverse implementations are, by and large, use secure transport connections to communicate with cloud servers instead of letting participating entities communicate directly. In this paper, we use the design and implementation of NDN Workspace, a web-based, multi-user collaborative app to showcase a new way to networking that supports many-to-many secure data exchanges among communicating entities directly. NDN Workspace users establish trust relations among each other, exchange URI-identified objects directly, and can collaborate through intermittent connectivity, all in the absence of cloud servers. Its data-centric design offers an exciting new approach to metaverse app development.

==> Makefile <==
PRJ = workspace

ifdef S
EXTRA = -synctex=1
endif

all : ${PRJ}.pdf

${PRJ}.pdf : *.tex *.tex *.bib
	pdflatex ${EXTRA} ${PRJ} && \
		(ls ${PRJ}.aux | xargs -n 1 bibtex) && \
		pdflatex ${EXTRA} ${PRJ} && pdflatex ${EXTRA} ${PRJ}

view : ${PRJ}.pdf
	open ${PRJ}.pdf &

clean:
	/bin/rm -f ${PRJ}.pdf *.toc *.aux *.bbl *.blg *.log *~* *.bak *.out *synctex.gz

distclean: clean
	/bin/rm -f ${PRJ}.pdf



==> datasec.tex <==
\subsection{Securely Data Directly}
\label{datasec}

NDN Workspace gives each application data object an URI-like name: \name{<username>/<workspace>/<seqNum>}, where \name{<username>} is the user identifier, \name{workspace} being the workspace to which users publish data, and \name{seqNum} being the sequence number of user publications in the same workspace.

\ty{have to talk about certificate naming here, moved to Yekta's text here} \yk{I agree. I think this paragraph is better here}
User certificates are also data objects with unique URI-like names: \name{<username>/KEY/<keyid>/self-sign/<version>},
% Every user in workspace holds a self-signed certificate. This self-signed certificate is used to cryptographically identify each user and the certificate itself can be identified by a unique URI-like name. The name for these self-signed certificates follow the format, \textit{/username/KEY/self-sign/v=version},
where \name{username} is the user identifier, \name{KEY} and \textit{self-sign} indicating the certificate is self-signed certificate, \textit{keyid} is the public key hash, and \textit{version} is the certificate version number.
As an example, 
\textit{alice@example.com/key/self-sign/v=1} would correspond to version one of the self-signed certificate owned by Alice, with the username \textit{alice@example.com}.

\ty{so that i) one user identifier can join multiple workspaces. ii) keys are retrievable and verifiable as a data object iii) enables policies, @Xinyu needs to talk about that}

\xm{Signing and encryption}
\ty{need to talk about signing and verification workflow, so we can create connection with \ref{wot}}

% Security bootstrapping enables users to produce SWO that carries document changes.
% The SWO namespace starts with each user's Workspace identity (discussed later in \S\ref{bootstrap}) and is followed by a sequence number, indicating the number of updates have been made by this user.
% Figure~\ref{fig:swo} gives an example of the Workspace naming convention, where Alice's changes are named sequentially under her \textit{meetings} identity prefix.
% % will ensure all users in it eventually seeing the same content in ``agenda.xml''.

% % Benefiting from named data rendezvous, retrieving key material is simplified to fetching yet another named data from the rendezvous point (\S\ref{rendezvous}).

% % \subsection{Document Consistency}
% % \label{sync}
% The \textit{meetings} workspace consists of multiple folders, each can contain multiple files.
% Workspace ensures that all users in \textit{meetings} eventually see the same agenda by representing this file hierarchy as a collection of shared data structures, referred to as \textit{Doc}.
% From Workspace's perspective, meeting organizer collaboration is driven by users making changes to the \textit{meetings} Doc.
% The file creation of ``agenda.xml'' is a change made to the file index structure, and the text Alice added to the agenda are a series of changes on text structure.
% By exchanging SWO on Doc changes, all users will get everyone else's updates made to the shared document, therefore hold the same view of the workspace.

% Workspace secures SWO by encrypting and signing them with keys, and keys themselves are also named and secured as SWO.
% % From the Workspace perspective, keys are certificates are also objects, which can be fetched directly by URI-like names.
% When Alice's Workspace instance signs SWO with her private keys, the signature can carry a URI-like key locator point to her certificate SWO.
% Data content are also encrypted by Alice's key with a key locator pointing to the encryption key SWO.

==> sync.tex <==
\subsection{Synchronizing Secured Data with URIs}
\label{sync}
\ty{@Varun?}

==> wot.tex <==
\subsection{Web of Trust Authentication}
\label{wot}
\ty{@Yekta, i will walk through this, changed my mind, focusing on email based name first, then talk about other names} \yk{So do you want to put that paragraph to its original place? Let's discuss during the meeting}



In addition to this self-signed certificate, users can issue certificates to other users as well as hold certificates issued by other users. This is necessary for establishing trust relationships between the users. Let's say Bob already trusts Alice and has learnt that Alice's username is \textit{alice@example.com} through out-of-band means. In that case, Bob would issue a certificate to Alice that carries Bob's signature and Alice's public key. The URI-like name for this certificate would follow a similar format, but change the \textit{self-sign} field in order to indicate this certificate is issued by another user. Following the example of Bob issuing a certificate to Alice, the name of this certificate would be \textit{14, where the signature comes from Bob's self signed certificate \textit{bob@example.com/key/self-sign/v=1}. With this certificate, whoever trusts Bob can authenticate Alice, establishing trust via a Web-of-Trust model. For example, let's say Jane and Bob has issued certificates to each other meaning they have established mutual trust. During this time, let's say Bob issues a certificate to Alice. As illustrated in figure \ref{fig:wot}, through the Web of Trust model, Jane can now authenticate Alice through his trust relationship with Bob.

In our current implementation, Bob learns Alice's username through out-of-band means in order to issue the certificate \textit{alice@example.com/key/bob-sign/v=1}. For the purpose of eliminating this out-of-band communication and providing a more seamless experience users, we plan to add functionalities where users authenticates each other by verifying name ownership.

\begin{figure}[h] \centering
\includegraphics[width=0.45\textwidth]{figures/wot.pdf} \caption{Bob and Jane has already established mutual authentication by issuing certificates to each other. After Bob issues a certificate to Alice, Bob now vouches for Alice's name ownership. So, Jane now trusts Alice by proxy.}\label{fig:wot}
\end{figure}


%Workspace users can mutually authenticate each other in two procedures: \textit{origin authentication} verifies the identity of the owner of a certificate, and \textit{endorsement} propagates the result of origin authentication.

% \paragraph{Origin Authentication:}
%To verify the identity of the a owner, one can make use of existing unique identifiers in the Internet.
%If the existing identity provider offers some resources modifiable by the owner of a identifier (\eg Tweet, Gist, DNS Records), the verifier (say Bob) can verify the ownership using some method similar to Let's Encrypt ACME~\cite{aas2019let} or Keybase~\cite{KeyBase}.
%For example, using authentication by email, Bob can send a random nonce to Alice via email, ask her to sign it and send back the signature.
%% to a channel that restricts write access only to the origin identity owner.
%In this way, Bob both verifies Alice's identifier (her email address) and obtains her public key.
% \lz{Please check correctness}

% \paragraph{Endorsement:}
%Having authenticated Alice, Bob signs Alice a endorsement certificate, thereby she can present Bob's endorsement when others try authenticating her.
%Eventually, every user in same workspace will have certificates signed by everyone else, and a fully meshed web of trust is formed in workspace. 

% \paragraph{Cloud Independence:}
%Workspace only uses origin identities for initial user security bootstrapping.
%After receiving an endorsement certificate, a user is bootstrapped into the web of trust and no need to communicate with today's authentication servers, and this web of trust runs completely independent from today's clouds.
%When there does not exist any trustworthy identity provider, one can use out-of-band channel to transmit the self-signed certificate directly to bootstrap a new user as a fallback.

%Although Workspace users mutually authenticate self-signed certificates, this approach differs from the concept of Web-of-Trust~\cite{golbeck2008weaving} with PGP~\cite{zimmermann1995official} keys, which focuses on endorsing self-signed certificates without unique semantic bindings.
%In order to collaborate, Workspace users already have out-of-band trust relations on their unique semantic identifiers (\eg emails, social media accounts), and mutual authentications leverage these pre-existing trust relations to authenticate and endorse self-signed certificates bound to their identifiers.
